On the Similarity between the Laplace and Neural Tangent Kernels

Recent theoretical work has shown that massively overparameterized neural networks are equivalent to kernel regressors that use Neural Tangent Kernels(NTK). Experiments show that these kernel methods perform similarly to real neural networks. Here we show that NTK for fully connected networks is closely related to the standard Laplace kernel. We show theoretically that for normalized data on the hypersphere both kernels have the same eigenfunctions and their eigenvalues decay polynomially at the same rate, implying that their Reproducing Kernel Hilbert Spaces (RKHS) include the same sets of functions. This means that both kernels give rise to classes of functions with the same smoothness properties. The two kernels differ for data off the hypersphere, but experiments indicate that when data is properly normalized these differences are not significant. Finally, we provide experiments on real data comparing NTK and the Laplace kernel, along with a larger class of{\gamma}-exponential kernels. We show that these perform almost identically. Our results suggest that much insight about neural networks can be obtained from analysis of the well-known Laplace kernel, which has a simple closed-form.

==> uci_exp.tex <==
%!TEX root = main.tex


In this section, we compare the performance of NTK with Laplace, Gaussian, and $\gamma$-exponential kernels. We present results on both small scale and large scale UCI tabular real datasets. The main goal of this section is to demonstrate- a) Results of Laplace are similar to those obtained by NTK, and b)~$\gamma$-exponential can achieve slightly better results as compared to NTK.

In section~\ref{small_uci}, we provide the results for small scale $90$ UCI datasets following the setup of~\cite{arora2019harnessing}. In section~\ref{large_uci}, we discuss the results for three large scale UCI datasets~(MillionSongs, SUSY, and HIGGS following the setup of~\cite{rudi2017falkon}. More details are provided in the appendix.

\subsubsection{Small Scale DataSets}\label{small_uci}

\cmt{
\begin{tiny}
\begin{figure*}[!htbp]
  \begin{minipage}[c]{0.5\textwidth}
    \includegraphics[height=4cm]{figures/wine-quality-white_ScaledKernel_True_N_4898_Dim_11.jpg}
  \end{minipage}\hfill
  \begin{minipage}[c]{0.5\textwidth}
    \caption{\small The plot of eigen values of different kernels for a UCI dataset~(wine-quality-white). The dotted red circle highlights the drastic difference in the decay rate of eigen values~(slope of the curve) of different kernels. NTK, Laplace, and Gaussian achieve best validation accuracies as $62.27$, $63.65$, $58.51$ and test accuracies as $67.25$, $68.97$, $62.74$. This demonstrates the richness of NTK and Laplace as compared to Gaussian.\abh{Ronen, please let me know if it makes sense. I can try to rewrite the caption but wanted to ensure this is what you wanted or something else?}
    \rb{On a second thought, we think we won't use this figure. I don't know if from this picture I could conclude that the Laplace kernel should be more similar to NTK than the Gaussian.}
    } \label{fig:compare_kernels_uciData}
  \end{minipage}
\end{figure*}
\end{tiny}
%Vertical alignment is controlled through optional argumants [c], [t] or [b] of minipage`
}


For appropriate comparison, we use the same set of $90$ small scale UCI datasets (less than $5000$ data points) as in~\cite{arora2019harnessing} for the evaluations. The results are provided in the Table~\ref{tab:scaled_kernel} for NTK, Laplace, Gaussian and $\gamma$-Exponential kernels. For completeness, we also cite the results for RF (Random forest, the top classifier identified in~\cite{fernandez2014we}) and neural networks from~\cite{arora2019harnessing}.\abh{Not sure, if we need Random forest at all, as already NTK established as Superior to RF in Arora paper}.

We report the same metrics as used in ~\cite{arora2019harnessing}: Friedman Ranking, Average Accuracy, P90/P95, and PMA. A superior classifier is expected to have lower Friedman rank and higher P90, P95, and PMA. Friedman Ranking is a ranking based metric to compare the performance of a classifier across multiple datasets~\cite{demvsar2006statistical} and reports the average ranking of a given classifier compared to other classifiers. P90/P95 denotes the fraction of datasets on which a classifier achieves
more than $90/95\%$ of the maximum achievable accuracy~\footnote{Maximum achievable accuracy is defined as the maximum accuracy among all the classifiers~\cite{fernandez2014we}}. PMA represents the percentage of maximum accuracy. A more detailed interpretation is provided in the appendix. \abh{To save some space, may be I can move this entire description (more or less) to the caption of the table itself ?}

From the Table~\ref{tab:standard_kernels}, one can observe that Laplace kernel results are the closest to NTK on all the metrics, and $\gamma$-Exponential outperforms all the classifiers including NTK on all the metrics as well.
\rb{Abhay, can you discuss the hyperparameter search for NTK vs. the other kernels?}\abh{Ronen, I thought that due to space limitation we will put that in the appendix, no?}
\rb{Just say over how many hyperparameters we searched, compared to NTK.}

\rb{Abay, also, can you merge Tables 2 and 3 (UCI)? Please order the rows as follows: H-$\gamma$-exp., $\gamma$-exp., H-Laplace, Laplace, H-Gaussian, Gaussian, NTK, NN, RF. Thanks}

\begin{table*}
        \centering
        %\begin{tiny}
        %\resizebox{\columnwidth}{!}{%
         %       \renewcommand{\arraystretch}{1.5}
\tiny{
\begin{tabular}{c|c|c|c|c|c}
\toprule
Classifier        & Friedman Rank  & Average Accuracy             & P90              & P95              & PMA       \\
\midrule

$\gamma$-Exponential               & \textbf{27.52} & \textbf{82.12\%$\pm$14.18\%} & \textbf{90.00\%} & \textbf{75.56\%} & \textbf{95.91\% $\pm$---\%} \\ 


NTK~\cite{arora2019harnessing}~\footnote{We report the number locally reproduced which are the same as in the paper~\cite{ntk_arora'}}               & 28.34 & 81.95\%$\pm$14.10\% & 88.89\% & 72.22\% & 95.72\% $\pm$5.17\% \\ 

Laplace                & 29.60 & 81.74\%$\pm$13.82\% & 88.89\% & 66.67\% & 95.53\% $\pm$---\% \\ 

Gaussian    & 32.66          & 81.46\% $\pm$ 14.83\%        & 84.44\%          & 67.77\% & 94.95\% $\pm$--\%          \\ 

NN (NTK init)~\cite{arora2019harnessing}     & 38.06          & 81.02\%$\pm$14.47\%          & 85.56\%          & 60.00\%          & 94.55\% $\pm$5.89\%          \\ 

% NN (He init)      & 40.97          & 80.88\%$\pm$14.96\%          & 81.11\%          & 65.56\%          & 94.34\% $\pm$7.22\%          \\ 

RF~\cite{arora2019harnessing}                & 33.51          & 81.56\% $\pm$13.90\%         & 85.56\%          & 67.78\%          & 95.25\% $\pm$5.30\%          \\ 

% Polynomial Kernel & 38.44          & 78.21\% $\pm$ 20.30\%        & 80.00\%          & 62.22\%          & 91.29\% $\pm$18.05\%         \\ 
\bottomrule
\end{tabular}
}
        %}
        \caption{\small Homogeneous Kernels.
                \label{tab:scaled_kernel}
}
%\end{tiny}
\end{table*}
%%appendix table, with Standard Kernels
\begin{table*}
        \centering
        %\begin{tiny}
        %\resizebox{\columnwidth}{!}{%
         %       \renewcommand{\arraystretch}{1.5}
\tiny{\begin{tabular}{c|c|c|c|c|c}
\toprule
Classifier        & Friedman Rank  & Average Accuracy             & P90              & P95              & PMA                   \\
\midrule

$\gamma$-Exponential               & 32.98 & 81.80\%$\pm$14.21\% & 85.56\% & 73.33\% & 95.49\% $\pm$---\% \\ 
NTK~\cite{arora2019harnessing}               & 28.34 & 81.95\%$\pm$14.10\% & 88.89\% & 72.22\% & 95.72\% $\pm$5.17\% \\ 
Laplace                & 33.28 & 81.12\%$\pm$14.16\% & 86.67\% & 65.56\% & 94.88\% $\pm$---\% \\ 
Gaussian    & 35.76          & 81.03\% $\pm$ 15.09\%        & 85.56\%          & 72.22\% & 94.56\% $\pm$8.22\%          \\
\bottomrule
\end{tabular}
        }
        \caption{\small Standard Kernels. \rb{Abhay, you seem to miss some stds in PMA.}
                \label{tab:standard_kernels}
}
%\end{tiny}
\end{table*}



%%%%%%%

\subsubsection{Large scale datasets}\label{large_uci}
We leverage FALKON~\cite{rudi2017falkon}, an efficient large scale kernel method to conduct large scale regression and classification tasks following the setup of~\cite{rudi2017falkon} on three datasets: MillionSongs~\cite{bertin2011million}, SUSY~\cite{CITE}, and HIGGS~\cite{CITE}. The results are reports in Table~\ref{table:largeData} for all the kernel methods including neural network results from ~\cite{baldi2014searching}. We searched for hyper-parameters based on a small validation dataset for all the methods and used the standard train/test partition provided on the UCI repository. From the Table~\ref{table:largeData}, one can notice that the NTK and Laplace perform similarly worse; Gaussian and $\gamma$-Exponential kernels perform slightly better than Gaussian. More details are provided in the appendix. \abh{Also, FALKON is an approximate efficient method for large scale kernel methods, not sure if should mention this ?}

\begin{table*}[!htbp]
%\vskip 0.15in
  \centering
  \begin{tiny}
  \begin{tabular}{c|c|c|c}
    \toprule
        & MillionSongs & SUSY & HIGGS \\
        \midrule
            \#Training Data                      &  $4.6\times10^5$    & $5\times10^6$ & $1.1\times 10^7$ \\
            \#Features                      & 90    & 18 & 28 \\
            Problem Type                      & Regression    & Classification & Classification \\
                        Performance Metric                      & MSE   & AUC & AUC \\
    \hline
    \hline
    
    
    $\gamma$-Exponential                      & \textbf{78.6417}    & 87.686 & \textbf{82.281} \\
    
    Laplace                      & 79.7941    & 87.670 & 81.995 \\
    
    NTK                    & 79.9666    & 87.673 & 82.089 \\
    
    Gaussian Kernel                     & 79.6255    & \textbf{87.689} & 81.967 \\
    
    \hline
    
    
    Neural Network \cite{baldi2014searching}  & - & 87.500    & 81.600 \\
    
    Deep Neural Network \cite{baldi2014searching} & -  & \textbf{87.900}$^{*}$    & \textbf{88.500}$^{*}$   \\
    
    \bottomrule
  \end{tabular} 
    %\vspace{0.1in}
     \caption{\small Large scale datasets. MSE~(Lower is better) and AUC~(Higher is better).}
     \label{table:largeData}
\end{tiny}
%\vskip -0.1in
\end{table*}

